A 7K Parameter Model for Underwater Image Enhancement based on Transmission Map Prior

Although deep learning based models for underwater image enhancement have achieved good performance, they face limitations in both lightweight and effectiveness, which prevents their deployment and application on resource-constrained platforms. Moreover, most existing deep learning based models use data compression to get high-level semantic information in latent space instead of using the original information. Therefore, they require decoder blocks to generate the details of the output. This requires additional computational cost. In this paper, a lightweight network named lightweight selective attention network (LSNet) based on the top-k selective attention and transmission maps mechanism is proposed. The proposed model achieves a PSNR of 97\% with only 7K parameters compared to a similar attention-based model. Extensive experiments show that the proposed LSNet achieves excellent performance in state-of-the-art models with significantly fewer parameters and computational resources. The code is available at https://github.com/FuhengZhou/LSNet}{https://github.com/FuhengZhou/LSNet.

==> main <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{1-jian2021underwater}
M.~Jian, X.~Liu, H.~Luo, X.~Lu, H.~Yu, and J.~Dong, ``Underwater image processing and analysis: A review,'' \emph{Signal Processing: Image Communication}, vol.~91, p. 116088, 2021.

\bibitem{2-shi2022integrating}
Z.~Shi, Y.~Wang, Z.~Zhou, and W.~Ren, ``Integrating deep learning and traditional image enhancement techniques for underwater image enhancement,'' \emph{IET Image Processing}, vol.~16, no.~13, pp. 3471--3484, 2022.

\bibitem{3-hitam2013mixture}
M.~S. Hitam, E.~A. Awalludin, W.~N. J. H.~W. Yussof, and Z.~Bachok, ``Mixture contrast limited adaptive histogram equalization for underwater image enhancement,'' in \emph{2013 International conference on computer applications technology (ICCAT)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2013, pp. 1--5.

\bibitem{4-ancuti2017color}
C.~O. Ancuti, C.~Ancuti, C.~De~Vleeschouwer, and P.~Bekaert, ``Color balance and fusion for underwater image enhancement,'' \emph{IEEE Transactions on image processing}, vol.~27, no.~1, pp. 379--393, 2017.

\bibitem{5-li2015underwater}
C.~Li and J.~Guo, ``Underwater image enhancement by dehazing and color correction,'' \emph{Journal of Electronic Imaging}, vol.~24, no.~3, pp. 033\,023--033\,023, 2015.

\bibitem{6-sathya2015underwater}
R.~Sathya, M.~Bharathi, and G.~Dhivyasri, ``Underwater image enhancement by dark channel prior,'' in \emph{2015 2nd International Conference on Electronics and Communication Systems (ICECS)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2015, pp. 1119--1123.

\bibitem{7-wen2013single}
H.~Wen, Y.~Tian, T.~Huang, and W.~Gao, ``Single underwater image enhancement with a new optical model,'' in \emph{2013 IEEE International Symposium on Circuits and Systems (ISCAS)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2013, pp. 753--756.

\bibitem{8-drews2013transmission}
P.~Drews, E.~Nascimento, F.~Moraes, S.~Botelho, and M.~Campos, ``Transmission estimation in underwater single images,'' in \emph{Proceedings of the IEEE international conference on computer vision workshops}, 2013, pp. 825--830.

\bibitem{9-perez2017deep}
J.~Perez, A.~C. Attanasio, N.~Nechyporenko, and P.~J. Sanz, ``A deep learning approach for underwater image enhancement,'' in \emph{Biomedical Applications Based on Natural and Artificial Computing: International Work-Conference on the Interplay Between Natural and Artificial Computation, IWINAC 2017, Corunna, Spain, June 19-23, 2017, Proceedings, Part II}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2017, pp. 183--192.

\bibitem{10-wang2017deep}
Y.~Wang, J.~Zhang, Y.~Cao, and Z.~Wang, ``A deep cnn method for underwater image enhancement,'' in \emph{2017 IEEE international conference on image processing (ICIP)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2017, pp. 1382--1386.

\bibitem{11-anwar2018deep}
S.~Anwar, C.~Li, and F.~Porikli, ``Deep underwater image enhancement,'' \emph{arXiv preprint arXiv:1807.03528}, 2018.

\bibitem{12-li2019underwater}
C.~Li, C.~Guo, W.~Ren, R.~Cong, J.~Hou, S.~Kwong, and D.~Tao, ``An underwater image enhancement benchmark dataset and beyond,'' \emph{IEEE transactions on image processing}, vol.~29, pp. 4376--4389, 2019.

\bibitem{13-guo2019underwater}
Y.~Guo, H.~Li, and P.~Zhuang, ``Underwater image enhancement using a multiscale dense generative adversarial network,'' \emph{IEEE Journal of Oceanic Engineering}, vol.~45, no.~3, pp. 862--870, 2019.

\bibitem{14-islam2020fast}
M.~J. Islam, Y.~Xia, and J.~Sattar, ``Fast underwater image enhancement for improved visual perception,'' \emph{IEEE Robotics and Automation Letters}, vol.~5, no.~2, pp. 3227--3234, 2020.

\bibitem{15-li2021underwater}
C.~Li, S.~Anwar, J.~Hou, R.~Cong, C.~Guo, and W.~Ren, ``Underwater image enhancement via medium transmission-guided multi-color space embedding,'' \emph{IEEE Transactions on Image Processing}, vol.~30, pp. 4985--5000, 2021.

\bibitem{16-fu2022uncertainty}
Z.~Fu, W.~Wang, Y.~Huang, X.~Ding, and K.-K. Ma, ``Uncertainty inspired underwater image enhancement,'' in \emph{European conference on computer vision}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2022, pp. 465--482.

\bibitem{17-peng2023u}
L.~Peng, C.~Zhu, and L.~Bian, ``U-shape transformer for underwater image enhancement,'' \emph{IEEE Transactions on Image Processing}, 2023.

\bibitem{18-yang2021laffnet}
H.-H. Yang, K.-C. Huang, and W.-T. Chen, ``Laffnet: A lightweight adaptive feature fusion network for underwater image enhancement,'' in \emph{2021 IEEE international conference on robotics and automation (ICRA)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2021, pp. 685--692.

\bibitem{19-lyu2022efficient}
Z.~Lyu, A.~Peng, Q.~Wang, and D.~Ding, ``An efficient learning-based method for underwater image enhancement,'' \emph{Displays}, vol.~74, p. 102174, 2022.

\bibitem{20-naik2021shallow}
A.~Naik, A.~Swarnakar, and K.~Mittal, ``Shallow-uwnet: Compressed model for underwater image enhancement (student abstract),'' in \emph{Proceedings of the AAAI Conference on Artificial Intelligence}, vol.~35, no.~18, 2021, pp. 15\,853--15\,854.

\bibitem{22-guo2023underwater}
C.~Guo, R.~Wu, X.~Jin, L.~Han, W.~Zhang, Z.~Chai, and C.~Li, ``Underwater ranker: Learn which is better and how to be better,'' in \emph{Proceedings of the AAAI conference on artificial intelligence}, vol.~37, no.~1, 2023, pp. 702--709.

\bibitem{23-jiang2023five}
J.~Jiang, T.~Ye, J.~Bai, S.~Chen, W.~Chai, S.~Jun, Y.~Liu, and E.~Chen, ``Five a $\^{}$\{$+$\}$ $ network: You only need 9k parameters for underwater image enhancement,'' \emph{arXiv preprint arXiv:2305.08824}, 2023.

\bibitem{24-zhu2023biformer}
L.~Zhu, X.~Wang, Z.~Ke, W.~Zhang, and R.~W. Lau, ``Biformer: Vision transformer with bi-level routing attention,'' in \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, 2023, pp. 10\,323--10\,333.

\bibitem{25-mittal2012making}
A.~Mittal, R.~Soundararajan, and A.~C. Bovik, ``Making a “completely blind” image quality analyzer,'' \emph{IEEE Signal processing letters}, vol.~20, no.~3, pp. 209--212, 2012.

\bibitem{26-wang2004image}
Z.~Wang, A.~C. Bovik, H.~R. Sheikh, and E.~P. Simoncelli, ``Image quality assessment: from error visibility to structural similarity,'' \emph{IEEE transactions on image processing}, vol.~13, no.~4, pp. 600--612, 2004.

\bibitem{27-yang2015underwater}
M.~Yang and A.~Sowmya, ``An underwater color image quality evaluation metric,'' \emph{IEEE Transactions on Image Processing}, vol.~24, no.~12, pp. 6062--6071, 2015.

\bibitem{28-panetta2015human}
K.~Panetta, C.~Gao, and S.~Agaian, ``Human-visual-system-inspired underwater image quality measures,'' \emph{IEEE Journal of Oceanic Engineering}, vol.~41, no.~3, pp. 541--551, 2015.

\bibitem{29-wang2019experimental}
Y.~Wang, W.~Song, G.~Fortino, L.-Z. Qi, W.~Zhang, and A.~Liotta, ``An experimental-based review of image enhancement and image restoration methods for underwater imaging,'' \emph{IEEE Access}, vol.~7, pp. 140\,233--140\,251, 2019.

\bibitem{30-he2010single}
K.~He, J.~Sun, and X.~Tang, ``Single image haze removal using dark channel prior,'' \emph{IEEE transactions on pattern analysis and machine intelligence}, vol.~33, no.~12, pp. 2341--2353, 2010.

\bibitem{31-rao2023deep}
Y.~Rao, W.~Liu, K.~Li, H.~Fan, S.~Wang, and J.~Dong, ``Deep color compensation for generalized underwater image enhancement,'' \emph{IEEE Transactions on Circuits and Systems for Video Technology}, 2023.

\bibitem{34-li2020underwater}
C.~Li, S.~Anwar, and F.~Porikli, ``Underwater scene prior inspired deep underwater image and video enhancement,'' \emph{Pattern Recognition}, vol.~98, p. 107038, 2020.

\bibitem{35-wang2019uwgan}
N.~Wang, Y.~Zhou, F.~Han, H.~Zhu, and J.~Yao, ``Uwgan: underwater gan for real-world underwater color restoration and dehazing,'' \emph{arXiv preprint arXiv:1912.10269}, 2019.

\bibitem{36-wang2021uiec}
Y.~Wang, J.~Guo, H.~Gao, and H.~Yue, ``Uiec\^{} 2-net: Cnn-based underwater image enhancement using two color space,'' \emph{Signal Processing: Image Communication}, vol.~96, p. 116250, 2021.

\bibitem{37-jaffe1990computer}
J.~S. Jaffe, ``Computer modeling and the design of optimal underwater imaging systems,'' \emph{IEEE Journal of Oceanic Engineering}, vol.~15, no.~2, pp. 101--111, 1990.

\bibitem{38-mcglamery1980computer}
B.~McGlamery, ``A computer model for underwater camera systems,'' in \emph{Ocean Optics VI}, vol. 208.\hskip 1em plus 0.5em minus 0.4em\relax SPIE, 1980, pp. 221--231.

\bibitem{39-schechner2005recovery}
Y.~Y. Schechner and N.~Karpel, ``Recovery of underwater visibility and structure by polarization analysis,'' \emph{IEEE Journal of oceanic engineering}, vol.~30, no.~3, pp. 570--587, 2005.

\bibitem{40-liu2020real}
R.~Liu, X.~Fan, M.~Zhu, M.~Hou, and Z.~Luo, ``Real-world underwater enhancement: Challenges, benchmarks, and solutions under natural light,'' \emph{IEEE transactions on circuits and systems for video technology}, vol.~30, no.~12, pp. 4861--4875, 2020.

\bibitem{41-li2019fusion}
H.~Li, J.~Li, and W.~Wang, ``A fusion adversarial underwater image enhancement network with a public test dataset,'' \emph{arXiv preprint arXiv:1906.06819}, 2019.

\end{thebibliography}

